Active Learning for Multilingual Semantic Parser

Current multilingual semantic parsing (MSP) datasets are almost all collected by translating the utterances in the existing datasets from the resource-rich language to the target language. However, manual translation is costly. To reduce the translation effort, this paper proposes the first active learning procedure for MSP (AL-MSP). AL-MSP selects only a subset from the existing datasets to be translated. We also propose a novel selection method that prioritizes the examples diversifying the logical form structures with more lexical choices, and a novel hyperparameter tuning method that needs no extra annotation cost. Our experiments show that AL-MSP significantly reduces translation costs with ideal selection methods. Our selection method with proper hyperparameters yields better parsing performance than the other baselines on two multilingual datasets.

==> 04_diff_to_previous_work.tex <==
There are multiple active learning works~\cite{duong2018active,ni2020merging,sen2020uncertainty} for monolingual semantic parsing. Differ from these works, our patent proposes the first active learning method for multilingual semantic parsing. 

Particularly, \citep{duong2018active,ni2020merging,sen2020uncertainty} assume there is an utterance pool in the target language. \citep{duong2018active,ni2020merging,sen2020uncertainty} select utterances from the utterance pool and annotate the logical forms for these utterances. This annotation procedure requires the annotators to have expert knowledge of the logical forms. However, the annotators who have expert knowledge are scarce. In contrast, our active learning method selects the utterances from existing semantic paring datasets. Afterwards, the annotators translate the utterances into target languages. The number of annotators with bilingual knowledge is much larger than those with expert knowledge of the logical forms. In addition, compared to previous active learning work, the annotation cost per utterance is much \textit{lower} in our method. We perform a rough estimation. Annotating the logical form for each utterance in SPIDER dataset~\cite{yu2018spider} is six minutes while translating one sentence in SPIDER from English to Chinese takes less than 1 minute. 

Second, our active learning designs a specific metric to decide which utterances should be selected. \cite{duong2018active,ni2020merging,sen2020uncertainty} also design several metrics to select utterances. Unlike their metrics, our metric tends to select utterances, the human translations of which \textit{fix} the bias and errors in the current dataset. But the metrics in previous works are not designed for this purpose. Therefore, with our metric, we could annotate much fewer utterances than the works~\cite{duong2018active,ni2020merging,sen2020uncertainty} that use other metrics. However, the parser using our metric can still perform comparably to the parsers that use metrics in~\citep{duong2018active,ni2020merging,sen2020uncertainty}.



%Active learning for deep semantic parsing
%Merging Weak and Active Supervision for Semantic Parsing
%Learning a Neural Semantic Parser from User Feedback
%Uncertainty and Traffic-Aware Active Learning for Semantic Parsing

%Active Learning for Node Classification: The Additional
%Learning Ability from Unlabelled Nodes

%Diverse mini-batch Active Learning

%Hierarchical Sampling for Active Learning

%Active Learning Using Pre-clustering

==> 05_method.tex <==


%In order to mitigate the two issues aforementioned, a small set of human translations can be included in the training set

In order to mitigate the performance loss caused by translation errors and translation bias, our active learning approach introduces extra human supervision to machine supervision when training the multilingual parser. Two major intuitions motivate our active learning approach:

\begin{enumerate}
    \item The error rate of human translations is much lower than the one of machine translations~\cite{freitag2021experts}. Therefore, training the multilingual parser on the correct translations can mitigate the training problems when training the multilingual parser on the noisy MT data with mistranslations.
    \item Increasing the lexical and morphological diversity of the training data could improve the generalization ability of the parsers. In addition, more human translations could ensure that the lexical distribution of the training data is closer to the human test set.
\end{enumerate}


In our active learning setting, we assume access to a well-trained black-box multilingual MT system, $g^{mt}(\cdot)$, and a semantic parsing dataset that includes utterances in a source language $l_s$ (e.g. English) paired with LFs, $\mathcal{D}_s = \{(\vx_{s}^i, \vy^i)\}_{i=1}^{N}$. Each utterance $\vx_{s}$ in $\mathcal{D}_s$ is translated into the utterance $\hat{\vx}_{t} = g^{mt}_{s\rightarrow t}(\vx_{s})$ in the target language $l_t$ by the MT system, $\hat{\mathcal{D}}_{t} = \{(\hat{\vx}^i_{t}, \vy^i)\}_{i=1}^{N}$. With a semantic parser initially trained on the the combination of source data and the MT data, $\mathcal{D} = \mathcal{D}_s \cup \hat{\mathcal{D}}_{t}$, the goal of our active learning method is to select a small set of utterances from the training data in the source language, $\tilde{\mathcal{D}}_s \in \mathcal{D}_s$, and translate the utterances in $\tilde{\mathcal{D}}_s$ to the target language by the human translators, $\mathcal{D}_t = g^{ht}_{s\rightarrow t}(\tilde{\mathcal{D}}_s)$. The selection criterion is based on the \textit{acquisition functions}, which score the source utterances. Following the conventional batch AL setting~\cite{duong2018active}, there are $Q$ rounds of selection. At $q$th round, AL selects utterances with a budget size of $K_q$.
%thus the size of $\mathcal{D}_{t,h} = \bigcup^{Q}_{q=1} \mathcal{D}^{q}_{t,h}$ is incrementally increasing. 
The detailed AL procedure iteratively performs the following steps at the $q$th query round:

\noindent\textbf{Step1}: Train the semantic parser $P_{\theta}(\vy|\vx)$ to convergence over the training data, $\mathcal{D}^{q} = \mathcal{D}_s \cup \hat{\mathcal{D}}_t \cup \mathcal{D}^{1:q-1}_t$, which is the combination of data in the source language $\mathcal{D}_s$, machine-translated data $\hat{\mathcal{D}}_t$ and the human-translated data from previous query rounds $\mathcal{D}^{1:q-1}_t = \bigcup^{q-1}_{i=1} \mathcal{D}^{i}_{t}$ if there are any.

\noindent\textbf{Step2}: With our active learning acquisition functions, select a subset $\tilde{\mathcal{D}}^{q}_s$ in size of $K_q$ from the source language data. The human annotators translate the utterances in $\tilde{\mathcal{D}}^{q}_s$ into the target language, $\mathcal{D}^{q}_t = g^{ht}_{s\rightarrow t}(\tilde{\mathcal{D}}^{q}_s)$.

\noindent\textbf{Step3}: Add the human-translated data into the training data, $\mathcal{D}^{1:q}_t = D^{1:q-1}_t \bigcup D^{q}_{t}$ and repeat Step1-Step3 until the $Q$ rounds of sample selection are performed.



%An LF $\vy = \{\vy_{s}^1,...,\vy_{s}^n\}$ can be further decomposed into a set of sub-structures, each of which $\vy_{s}^n = (\vv_{s}^{n}, \ve_{s}^{n})$ is constructed by the subset of the node set $\vv_{s}^{n} \subseteq \vv$ and the edges linking the nodes $\ve_{s}^{n} \subseteq \vv_{s}^{n} \times \vv_{s}^{n} $.

%Each task $\mathcal{T}^{(k)}$ includes its own training/validation/test set ($\mathcal{D}^{(k)}_{train}$,$\mathcal{D}^{(k)}_{valid}$,$\mathcal{D}^{(k)}_{test}$), each of which is a set of utterance-LF pairs $(\mathcal{X}^{(k)}, \mathcal{Y}^{(k)})$. The \textit{boundaries} between tasks are defined by \textit{task descriptors}~\cite{lopez2017gradient}, which provides contextual information about examples $(\mathcal{X}^{(k)}, \mathcal{Y}^{(k)})$ in each task. For example, the descriptors might describe that each task belongs to a distinct domain, or the questions $\mathcal{X}^{(k)}$ in each task are in a unique set of types or querying about a distinct set of cities. The node set $\mathcal{V}^{(k)} = \mathcal{V}^{(k)}_{s} \cup \mathcal{V}_g $ in the LFs $\mathcal{Y}^{(k)}$ of each task $\mathcal{T}^{(k)}$ can be further divided into task-specific nodes $\mathcal{V}^{(k)}_{s}$ and task-general nodes $\mathcal{V}_{g}$. The task-specific nodes $\mathcal{V}^{(k)}_{s}$ only exist in $k$-th task while the task-general nodes $\mathcal{V}_{g}$ are shared across different tasks \reza{among tasks seen so far?}. 
%As an example in Table , the nodes, "" and "", in LFs from two different tasks, "" and "", are distinct in each task, while the rest nodes are shared by two LFs. 
%Task-specific nodes $\mathcal{V}_{s}$ usually possess semantics related to descriptors, such as entities in each domain, question types or city names.
% to do a table showing two LFs from different tasks.
\subsection{Acquisition Functions} 
%\textbf{Hypothesis:} \textit{To mitigate the translation bias and error problems in the overall dataset, we should select the diversified and representative source utterances in the training set that have biased and erroneous translations.}
%The acquisition functions are designed based on our intuitions to mitigate the translation errors and translation bias. Formally, the active learning problem is to sample and annotate a small set of examples to minimize the future risk~\cite{}. Since this target is difficult to achieve, many current works reformulate this problem into sampling the examples that could maximize the total risk of the models after annotation. In our problem, the objective when we select each example turns to:

% \begin{small}
% \begin{align}
%     \argmax_{\vx_s,\vy}\iint R(\pi_{\theta}(\vx_{t}), \vy)p(\vx_t,\vx_s,\vy)\,d\vx_t \,d\vy
% \end{align}
% \end{small}

%\noindent\ignorespaces where $p_{D}(\vx_t,\vx_s,\vy)$ is the distribution of the the training data $D$, which includes source language data, MT translated data and human translated data. With a simple Bayesian factorization,

% \begin{small}
% \begin{align}
%     p(\vx_t,\vx_s,\vy) = \frac{p(\vx_t,\vx_s,\vy)}{p_{D}(\vx_t,\vx_s,\vy)}p_{D}(\vx_t,\vx_s,\vy)
% \end{align}
% \end{small}

% \noindent\ignorespaces If we assume the $p_{D}(\vx_s,\vy)$ is the same as the true distribution of the source language data since $\vs_s$ is the human data, we can see the objective becomes:
% \begin{small}
% \begin{align}
% \label{eq:obj}
%     \argmax_{\vx_s,\vy}\iint R(\pi_{\theta}(\vx_{t}),\vy) \frac{p(\vx_t|\vx_s,\vy)}{p_{D}(\vx_t|\vx_s,\vy)}p_{D}(\vx_t,\vx_s,\vy)\,d\vx_t \,d\vy
% \end{align}
% \end{small}

%Given our hypothesis to mitigate translation bias and errors, we derive four acquisition functions for selecting the utterances. Then, we aggregate the four acquisition functions to acquire their joint benefits. In each AL round, the utterances with the highest acquisition scores are selected in each round.

\paragraph{Lexical Diversity} 

%The term $\frac{p(\vx_t|\vx_s,\vy)}{p_{D}(\vx_t|\vx_s,\vy)}$ in Eq. \ref{eq:obj} implys that the $\vx_s$ with the largest translation bias should be selected. However, true distribution $p(\vx_t|\vx_s,\vy)$ is usually unknown. Therefore, here we made an assumption $p(\vx_t|\vx_s,\vy)$ is in an uniform distribution since the human translations are more diversified.
We assume an empirical conditional distribution, $P_{e}^{q}(X_t|\vx_s)$, for each utterance $\vx_s$ in $\mathcal{D}_{s}$ at $q$th selection round, where $X_t$ is the random variable for the target utterances $\vx_t$. The empirical conditional distribution is considered as an mixture of human translation distribution and the machine translation distribution, $P_{e}^{q}(X_{t}|\vx_s) = \lambda^{\vx_s}_{q} P_{ht}(X_{t}|\vx_s) + (1-\lambda^{\vx_s}_{q})P_{mt}(X_{t}|\vx_s)$, where $\lambda_{q}^{\vx_s}$ is a coefficient between 0 and 1. 
%After annotation of $x_s$ at each round, $P_{e}^{q}(\mathcal{X}_{t}|\vx_s)$ is more close to the human translation distribution

%over the source and target utterances in the training data, $\mathcal{D}^{q}$ at $q$th round.
Intuitively, the $\vx_s$ with the most biased translations should be the one with the most skewed empirical conditional distribution. Therefore, we measure the translation bias by calculating the entropy of the empirical conditional distribution, $H(P_{e}^{q}(\mathcal{X}_{t}|\vx_s))$, and select the $\vx_s$ with the lowest entropy. Since the number of $\mathcal{X}_{t}$ is exponentially large, it is intractable to directly calculate the entropy. Following ~\cite{settles-craven-2008-analysis}, we adopt two approximation strategies, \textit{N-best Sequence Entropy} and \textit{Maximum Confidence Score}, to approximate the entropy.



%\noindent\ignorespaces where $\mathcal{N} = \{\vx_{t}\}^{N}_{1}$ are the $N$ best hypothesis sampled from the empirical distribution $P_{e}^{q}(\mathcal{X}_{t}|\vx_s)$. $P_{e}^{q}(\vx_t|\vx_s)$ is re-normalized since $\mathcal{N}$ is only a subset of $\mathcal{X}_{t}$.

%Though we could use a seq2seq model to estimate each $p_{D}(\vx_t|\vx_s,\vy)$, we adopt the IBM1 model~\cite{} to reduce the model training time. Heuristically, the more probable translations the $\vx_s$ has, the less likely it will be selected given this term. More probable translations also imply that $\vx_s$ have more diversified translations than the others.

%A direct way to estimate the empricial distribution $p(\vx_t|\vx_s)$ is to use a machine translation model. However,  Instead, we estimate $\sum_{\vy \in \mathcal{Y}} p(\vx_t|\vy) p(\vy|\vx_{s})$. Since $p(\vy|\vx_{s})$ is deterministic, we use a Seq2Seq model to estimate $p(\vx_t|\vy)$.


%\noindent\textit{Maximum Confidence Score (MCS):}

\begin{small}
\begin{align}
     \phi_b(\vx_s, \vy) & = -\frac{1}{|\vy|} \sum_{y_i \in \vy} H(p(\vx_{s}|y_{i})) \\
     s.t. \vy & = \argmax_{\vy} p(\vy|\vx_s)
 \end{align}
 \end{small}


\noindent\ignorespaces A direct way to estimate the empirical distribution $P_{e}^{q}(\mathcal{X}_t|\vx_s)$ is to train a machine translation model (i.e. a statistical model or a neural Seq2Seq model) on the translation pairs $(\vx_s, \vx_t)$ in $\mathcal{D}^{q}$. However, since empirical distribution is the mixture of two complicated distributions, the distribution of human translation and the distribution of the machine translation service., $\mathcal{D}^{q}$ is too small to train a decent translation model that estimates the empirical distribution. Instead, we use a bayesian factorization trick that factorizes $P_{e}^{q}(\vx_{t}|\vx_s) = \sum_{\vy \in \mathcal{Y}} P_{e}^{q}(\vx_t|\vy) P_{e}^{q}(\vy|\vx_{s})$. Since $P_{e}^{q}(\vy|\vx_{s})$ is deterministic, we only need to estimate $P^{q}_{e}(\vx_t|\vy)$. The intuition behind is straightforward. The more diversified data should have more lexically and morphologically diversified utterances per each LF. Note that if we use this factorization, all $x_s$ that share the same LF will have same scores. However, we found the bias acquisition functions using this factorization performs much better. 

We use the lightweight Seq2Seq model to estimate $P_{e}^{q}(X_t|\vx_s)$, which only takes around 30s on \geo to train the model. Ideally, every time a new source utterance $\vx_s$ is selected, $P_{e}^{q}(X_t|\vx_s)$ should be re-estimated. However, we only re-estimate $P_{e}^{q}(X_t|\vx_s)$ once at the beginning of each selection round to reduce the training cost.
%where $\mathcal{V}_{t}$ is the vocabulary extracted from training set $\mathcal{D}$ in the target language
\paragraph{Translation Error.} 
Similar to~\cite{haffari-etal-2009-active}, we leverage back-translations to measure the translation error. If machine translation quality for one source utterance $\vx_s$ is good enough, the semantic parser should be confident in its back-translation as well. In other words, if the parser is not confident, $\vx_s$ most likely has translation errors. Therefore, we measure the translation error for each $\vx_s$ with the expectation of parsers' negative confidence in the back-translations of the source utterance, $\mathbb{E}_{P^{q}_{e}(\mathcal{X}_{t}|\vx_s)}[-\log(P^{q}_{\theta}(\vy_{\vx_s}|g_{t \rightarrow s}^{mt}(\vx_t)))]$, where $\vy_{\vx_s}$ is the corresponding LF of $\vx_s$, $g_{t \rightarrow s}^{mt}$ is the back-translation model and $P^{q}_{\theta}$ is the parser trained at $q$th round. To approximate the expectation, we apply two similar strategies as mentioned in \textit{Translation Bias}.
%The maximize the risk of the parser over the $\vx_t$, $R(\pi_{\theta}(\vx_{t}),\vy)$, one direct way is to select the examples in the source language with translation errors. Since it is difficult to measure the translation error between $\vx_s$ and its corresponding MT translation $\vx_{t,m}$. We provide an indirect way to measure the translation error using the trained semantic parser:

\noindent\textit{N-best Sequence Expected Error:}

\begin{small}
\begin{align}
    \phi_e(\vx_s, \vy) & = -\sum_{\vx_t \in \mathcal{N}_{\vy_{\vx_s}}} P_{e}^{q}(\vx_t|\vx_s) \log P^{q}_{\theta}(\vy_{\vx_s}|g_{t \rightarrow s}^{mt}(\vx_t)) 
\end{align}
\end{small}

\noindent\ignorespaces where $\mathcal{N}_{\vy_{\vx_s}}$ is the set of utterances in $\mathcal{D}^q$ in target language that share the same LF $\vy_{\vx_s}$ with $\vx_s$. We only back-translate utterances in $\mathcal{D}^q$ to reduce the cost of back-translations.

%where $\vx'_s = g^{-1}_{mt}(\vx_t)$ is the back-translation of $\vx_s$ with $\vx_{t} = g_{mt}(\vx_s)$ as its bridge utterance, $\mathcal{M}_{\vy}$ includes $\vx_t$ that shares the same $\vy$ with $\vx_s$. A direct way to estimate the empirical distribution $p(\vx_t|\vx_s)$ is to use a machine translation model. However,  Instead, we factorize $\sum_{\vy \in \mathcal{Y}} p(\vx_t|\vy) p(\vy|\vx_{s})$. We use a Seq2Seq model to estimate $p(\vx_t|\vy)$. We assume that if the translation is not correct, the parser will not be able to parse its corresponding back-translation correctly.

\noindent\textit{Maximum Error:}

\begin{small}
\begin{align}
    \phi_e(\vx_s, \vy) & = - \log P_{\theta}(\vy|\vx_s)) \\
\end{align}
\end{small}

\noindent\ignorespaces The $P^{q}_{e}(\mathcal{X}_{t}|\vx_s)$ is the same translation model used for \textit{Translation Bias}.

%where $\vx_t$ is obtained by $\vx_t = \argmax_{\vx_t} p_{E}(\mathcal{X}_{t}|\vx_s)$. We don't need to train any model here since $\argmax_{\vx_t} p_{E}(\mathcal{X}_{t}|\vx_s)$ is already provided by MT model, $\vx_t = g_{mt}(\vx_s)$. After annotation, the $\argmax_{\vx_t} p_{E}(\mathcal{X}_{t}|\vx_s)$ is presumed to be the human translation.
%Shannon's diversity index

\paragraph{Semantic Density.}
Empirically, the translations of the most representative source utterances influence the parsing performance the most. Therefore we desire to mitigate the translation error and bias for the most representative source utterances, and the utterances should be selected from the dense regions in the semantic space. In our work, we use kernel density estimation~\cite{botev2010kernel} with the exponential kernel to estimate $P(\vx_s)$ while other density estimation methods could also work. The feature of $\vx_s$ for density estimation is generated by averaging the contextual sequence representations of the pre-trained language model used in the encoder of the multilingual semantic parser. The density is re-estimated at the beginning of each query selection round.
\begin{equation}
    \phi_s(\vx_s) = \log P(\vx_s)
\end{equation}

\paragraph{Semantic Diversity.} The usage of the semantic diversity function is twofold. First, it prevents the AL method from selecting similar utterances. Second, semantic diversity could enrich the lexical diversity as well.

\begin{small}
\begin{align}
    \phi_d(\vx_s) =     
    \begin{cases}
      0 & \text{if $c(\vx_s) \notin \cup^{|\mathcal{S}|}_{i=1} c(\vx^{i}_s)$}\\
      -\infty & \text{Otherwise}
    \end{cases}
\end{align}
\end{small}

We adopt a diversify strategy as in ~\cite{ni2020merging,nguyen2004active} that uses the clustering algorithm to diversify the selected utterances. We use a clustering algorithm (i.e. k-means) to partition the source utterances into $|\mathcal{S}|$ clusters and ensure we will select at most one utterance from each cluster. Notice the number of clusters should be greater than or equal to the total budget size $|\mathcal{S}| \geq \sum^{q}_{i=1}K_{i}$ until current selection round. The clusters are re-estimated every round as well. To ensure the optimal exploration of semantic spaces across different query rounds, we adopt the Incremental K-means~\cite{liu2020active}. At each new round, Incremental K-means consider the selected utterances as the fixed clustering centers and learn the new clusters conditioned on the fixed centers.
\paragraph{Aggregated Acquisition.}
We aggregate the four acquisition functions into one acquisition function.
\begin{align}\nonumber
\label{eq:sample}
    & \phi_{A}(\vx_s) = \sum_{k}\alpha_{k} \phi_{k}(\vx_s) 
    %s.t. & c(\vx_s,\vy) \notin \cup^{|\mathcal{L}|}_{i=1} c(\vx^{i}_s,\vy)
\end{align}
\noindent where $\alpha_{k}$ is the coefficient. Each $\phi_{k}(\vx_s)$ is standardized using quantiles information~\cite{}. Given the approximation strategies we used for \textit{Translation Bias} and \textit{Translation Error}, we provide two types of aggregations, \amspnbest and \amspmax. \amspnbest uses \textit{N-best Sequence Entropy} and \textit{N-best Sequence Expected Error}. \amspmax uses \textit{Maximum Confidence Score} and \textit{Maximum Error}.
%\subsection{Hyperparameter Tuning}

==> tab-abl-diversity_error.tex <==
\begin{table}[ht]
    \vspace{-2mm}
\centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{|c|cccc|cccc|c|}
    \toprule
     Metric &  \bias & \error & \density & \diversity &  - \bias & - \error & - \density & - \diversity & \amspnbest  \\
      \midrule
          Error$\uparrow$ &   &  &  &  &  &  &  & & \\
     \hline
    BLEU$\uparrow$ &  - & - & - & - & 19.67 & - & - & - & 19.51 \\
\hline
    Self-BLEU$\downarrow$ & -  & - & - & - & 78.44 & - & - & - &77.80 \\
  MTLD$\uparrow$ & - &  -  & -  & - & 23.86 & - & - & - & 23.86   \\
        \hline
 Simpson Index$\downarrow$ & - & - & - & - &93.24 & - & - & -  & 93.15 \\
    \bottomrule
  \end{tabular}%
  }
    \caption{The scores of three metrics to measure the bias of the human (HT) and machine (MT) translations in \geo and \nlmap in German (De), Thai (Th) and Greek (El). '-' means Simpson Index does not apply to Thai. \vspace{-2mm}}
  \label{tab:abl_diversity_error}
  \vspace{-2mm}
\end{table}

==> tab-abl-diversity_error_back.tex <==
\begin{table}[ht]
    \vspace{-2mm}
\centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{|c|cccc|cccc|c|}
    \toprule
     Metric &  \bias & \error & \density & \diversity &  - \bias & - \error & - \density & - \diversity & \amspnbest  \\
      \midrule
          Error$\uparrow$ &   &  &  &  &  &  &  & & \\
     \hline
    BLEU$\uparrow$ &  20.27 & 20.13 & 20.59 & 20.04 & 21.46 & 20.20 & 19.69 & 20.11 & 20.72 \\
\hline
    Self-BLEU$\downarrow$ & 74.59  & 74.12 & 77.88 & 76.02 & 76.16 & 76.19 & 75.79 & 79.42 &76.01 \\
  MTLD$\uparrow$ & 35.43 &  35.28  & 34.41  & 34.89 & 35.07 & 34.25 & 34.98 & 35.74 & 35.23   \\
        \hline
 Simpson Index$\downarrow$ & 92.93 & 92.61 & 92.34 & 93.21 &93.00 & 93.15 & 92.83 & 95.65  & 92.91 \\
    \bottomrule
  \end{tabular}%
  }
    \caption{The scores of three metrics to measure the bias of the human (HT) and machine (MT) translations in \geo and \nlmap in German (De), Thai (Th) and Greek (El). '-' means Simpson Index does not apply to Thai. \vspace{-2mm}}
  \label{tab:abl_diversity_error}
  \vspace{-2mm}
\end{table}

==> tab-bias.tex <==
\begin{table}[ht]
    \vspace{-2mm}
\centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{|c|cc| cc| cc|cc|}
    \toprule
    \multirow{2}{*}{Metrics} &
      \multicolumn{2}{c|}{\geode} &
      \multicolumn{2}{c|}{\geoth} &
      \multicolumn{2}{c|}{\geoel} &
      \multicolumn{2}{c|}{\nlmapde}\\
     & HT& MT & HT& MT & HT& MT & HT & MT  \\
      \midrule
    BLEU$\uparrow$ &  31.10 & 18.81 & 56.45 & 20.52 & 41.84 & 24.12 & 20.56 & 19.70 \\
\hline
    %Self-BLEU$\downarrow$ &  - & - & - & - & - & - & - & - \\
  MTLD$\uparrow$ & 26.02&  22.50  & 20.74  & 19.07 & 28.16& 27.08 & 44.80&42.38    \\
        \hline
 %Simpson Index$\downarrow$ & 92.57&  93.74 & - & - &99.91 & 100.00 & 94.80&  95.11\\
    \bottomrule
  \end{tabular}%
  }
    \caption{The scores of three metrics to measure the bias of the human (HT) and machine (MT) translations in \geo and \nlmap in German (De), Thai (Th) and Greek (El). %'-' means Simpson Index does not apply to Thai. 
    \vspace{-2mm}}
  \label{tab:bias_analysis}
  \vspace{-2mm}
\end{table}

==> tab-correctness.tex <==
\begin{table}[t]
    % \vspace{-1mm}
\centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{|c||cccc|}
    \toprule
   
      & \geode  & \geoel & \geoth & \nlmapde   \\
       \midrule \midrule
     BT Error Rate & 11\% & 12\% &  10\% &10\% \\
                
    \bottomrule
  \end{tabular}%
  }
    \caption{The semantic-change rate between the English utterances in \geo and \nlmap and their corresponding back-translations using German (De), Thai (Th) and Greek (El) as the bridge languages. \vspace{-3mm}}
  \label{tab:change_rate}
    
\vspace{-3mm}
\end{table}

==> tab-diversity_error.tex <==
\begin{table*}[ht]
\centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{|c|c|ccccccc|cc|c|}
    \toprule
     Metric & No HT & \rand & \cluster & \csse & \rttl & \lcsfw & \lcsbw & \traffic & \amspnbest & \amspmax & \oracle  \\
      \midrule
          BT Error Rate$\uparrow$ & - & 11\%  & 14\% & 11\% & 21\% & \textbf{22\%} & 8\% & 14\% & 17\% & 18\% & - \\
     \hline
          \hline
    BLEU$\uparrow$ & 18.81 &  26.90 & 27.65 & 22.41 & 25.36 & 22.70 & 23.31 & 26.63 & \textbf{32.33} & 31.94 & 31.10 \\
\hline
  MTLD$\uparrow$ & 22.50 & 23.79$\ddagger$ &  23.32  & 22.65  & 22.89 & 23.00 & 22.27& 23.42 & \textbf{23.93} & 23.78  & 24.23 \\
          \hline
    \bottomrule
  \end{tabular}
  }
    \caption{The scores of metrics to measure the error rate of the back-translations of the selected utterances and the bias of the training set in \geode at the final AL round. All lexical diversity results compared with \amspnbest are statistically significant in t-test~\cite{kim2015t} except for MTLD of \rand. \vspace{-2mm}}
  \label{tab:main_diversity_error}
  \vspace{-2mm}
\end{table*}


 %Simpson Index$\downarrow$ & 93.74 & 93.65 & 93.57 & 93.38 & \textbf{92.10} &92.71 & 94.43 & 93.73&  93.28 & 93.30 & 92.81\\
     %Self-BLEU$\downarrow$ &  78.39 & 79.30 & 78.16 & 77.99 & \textbf{74.93} & 84.57 & 81.26 & 76.01 & 76.37 \\

==> tab-diversity_error_back.tex <==
\begin{table}[ht]
    \vspace{-2mm}
\centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{|c|ccccccc|cc|}
    \toprule
     Metric & \rand & \cluster & \csse & \rttl & \lcsfw & \lcsbw & \traffic & \amspnbest & \amspmax  \\
      \midrule
          Error$\uparrow$ & 11\%  & 14\% & 11\% & 21\% & \textbf{22\%} & 8\% & 14\% & 17\% & 18\% \\
     \hline
    BLEU$\uparrow$ &  20.07 & 20.38 & 19.56 & 20.05 & 18.79 & 18.71 & 19.22 & 20.72 & \textbf{20.91} \\
\hline
    Self-BLEU$\downarrow$ &  78.39 & 79.30 & 78.16 & 77.99 & \textbf{74.93} & 84.57 & 81.26 & 76.01 & 76.37 \\
  MTLD$\uparrow$ & 34.07 &  33.61  & 34.14  & 34.96 & 34.22 & 33.32 & 33.79 & \textbf{35.23} & -    \\
        \hline
 Simpson Index$\downarrow$ & 93.41 & 93.32 & 93.13 & \textbf{91.82} &92.48 & 94.25 & 93.51&  92.91 & 93.06\\
    \bottomrule
  \end{tabular}%
  }
    \caption{The scores of three metrics to measure the bias of the human (HT) and machine (MT) translations in \geo and \nlmap in German (De), Thai (Th) and Greek (El). '-' means Simpson Index does not apply to Thai. \vspace{-2mm}}
  \label{tab:main_diversity_error}
  \vspace{-2mm}
\end{table}
